Prune Wisely, Reconstruct Sharply: Compact 3D Gaussian Splatting via Adaptive Pruning and Difference-of-Gaussian Primitives

Recent significant advances in 3D scene representation have been driven by 3D Gaussian Splatting (3DGS), which has enabled real-time rendering with photorealistic quality. 3DGS often requires a large number of primitives to achieve high fidelity, leading to redundant representations and high resource consumption, thereby limiting its scalability for complex or large-scale scenes. Consequently, effective pruning strategies and more expressive primitives that can reduce redundancy while preserving visual quality are crucial for practical deployment. We propose an efficient, integrated reconstruction-aware pruning strategy that adaptively determines pruning timing and refining intervals based on reconstruction quality, thus reducing model size while enhancing rendering quality. Moreover, we introduce a 3D Difference-of-Gaussians primitive that jointly models both positive and negative densities in a single primitive, improving the expressiveness of Gaussians under compact configurations. Our method significantly improves model compactness, achieving up to 90\% reduction in Gaussian-count while delivering visual quality that is similar to, or in some cases better than, that produced by state-of-the-art methods. Code will be made publicly available.

==> sec/5_Ablation.tex <==
\section{Ablation Study}

We isolate our contributions using a set of modified architectures. Start with the 3DGS backbone, with 100\% primitives in the first row. We first use the refinement interval Regulation (RIR) as V1 to prune 90\% of primitives, and then, at each step, prune the same number of primitives based on opacity rank. In V2, the Dynamic Pruning Ratio Adjustment(DPRA) is integrated to tune the number of pruning primitives at each step. The Spatio-spectral Pruning Score (SPS) is adopted to replace opacity to measure per-primitive importance in the 3DGS model in V3. Finally, we introduce a novel 3D-DoG primitive into the architecture to formulate our method. 

\autoref{tab:ablation} mainly compares visual quality metrics between different model variants. As the method scales, the performance of the model with 10\% parameter steadily approaches that of the entire 100\% model, demonstrating the effectiveness and general superiority of our architecture.

\autoref{tab:ablation2} further discusses the contributions of our approaches to the efficiency of 3DGS. Compared to the original 3DGS, V1 achieves a 2$\times$ improvement in FPS and a training acceleration of approximately 1.29$\times$, while V2 further reduces the train time. V3 basically stays the same as V2 in terms of efficiency. Finally, our approach suffers from a slight degradation in training speed and FPS due to the overhead introduced by 3D-DoG primitives. 
\begin{table}[h]
    \centering
    \small
    \setlength{\tabcolsep}{3pt}
    \begin{tabular}{l|cccc |ccc}
    \multicolumn{1}{l}{}  &\multicolumn{4}{c}{\textbf{Components}} & \multicolumn{3}{c}{\textbf{Metrics}}  \\
    Variant & RIR  & DPRA  & SPS  & 3D-DoG& PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$  \\
    \hline
     3DGS &\xmark  & \xmark & \xmark &\xmark & 27.47 & 0.826 & 0.201  \\
    V1 &\cmark  & \xmark & \xmark & \xmark & 22.93  &  0.805 & 0.291\\
    V2 &\cmark  & \cmark & \xmark & \xmark & 22.71  &  0.798 & 0.306 \\
    V3 &\cmark  & \cmark & \cmark & \xmark & 26.99  &  0.771 & 0.299\\
     Ours &\cmark & \cmark & \cmark & \cmark & \cellcolor{lightred}27.16  & \cellcolor{lightred}0.789  & \cellcolor{lightorange}0.285\\
    \end{tabular}%
    \caption{The reconstruction performance of different variants. We report the average PSNR, SSIM, and LPIPS scores for the Mip-NeRF360 dataset with 3DGS as the backbone. $\uparrow$ refers larger values are better while $\downarrow$ is opposite.}
    \label{tab:ablation}
    %\vspace{-0.5cm}
\end{table}

\begin{table}[h]
    \centering
    \small
    \setlength{\tabcolsep}{3pt}
    \begin{tabular}{l|cccc | cc}
     \multicolumn{1}{l}{}  &\multicolumn{4}{c}{\textbf{Variants}}&\multicolumn{2}{c}{\textbf{Metrics}}  \\
     Variant &RIR  & DPRA  & SPS  & 3D-DoG& Time$\downarrow$ & FPS$\uparrow$   \\
    \hline
     3DGS & \xmark  & \xmark & \xmark &\xmark & 17m1s  & 0.826   \\
     V1 &\cmark  & \xmark & \xmark & \xmark & 13m56s  &  0.805 \\
    V2 &\cmark  & \cmark & \xmark & \xmark & \cellcolor{lightyellow}13m11s  &  0.798  \\
    V3   &\cmark  & \cmark & \cmark & \xmark & \cellcolor{lightred}13m10s  &  0.771 \\
     Ours &\cmark & \cmark & \cmark & \cmark & \cellcolor{lightorange}13m48s  &\cellcolor{lightorange}0.789  \\
    \end{tabular}%
    \caption{The efficiency evaluation of different variants. We report the training time, rendering FPS for the Mip-NeRF360 dataset with 3DGS as the backbone.}
    \label{tab:ablation2}
    \vspace{-0.5cm}
\end{table}
